Analyzing and Interpreting Neural Networks for NLP: A Report on the First BlackboxNLP Workshop

The EMNLP 2018 workshop BlackboxNLP was dedicated to resources and techniques specifically developed for analyzing and understanding the inner-workings and representations acquired by neural models of language. Approaches included: systematic manipulation of input to neural networks and investigating the impact on their performance, testing whether interpretable knowledge can be decoded from intermediate representations acquired by neural networks, proposing modifications to neural network architectures to make their knowledge state or generated output more explainable, and examining the performance of networks on simplified or formal languages. Here we review a number of representative studies in each category.

==> leave_out.tex <==
\section{Papers with marginal value or relevance, or those which don't fit the general themes we cover here}

\citeA{W18-5451}: this is a visualization tool for analyzing a sequence to sequence model.

In this work, we present the visual analysis tool SEQ2SEQ-VIS that allows interaction and ”what if”-style exploration of trained seq2seq models through each stage of the translation process. The aim is to identify which patterns have been learned, to detect errors within a model, and to understand the model through counterfactual scenarios. In order to investigate the origin of an error within a seq2seq model, we separate errors within each translation stage into the following categories: (1) representation errors, in which an encoder or decoder misrepresent a word within a given context (2) alignment errors, in which the attention focuses on the wrong word, and (3) decoding errors, in which the prediction assigns a wrong probability distribution over words, or the beam search fails to include the correct solution. We define three steps within an analysis that aim to understand the prediction process, understand how an output relates to training data, and examine causal relationships between inputs and outputs. Examine Model Outputs: SEQ2SEQVIS shows a separate visual representation for the output of each stage of the seq2seq pipeline. Connect Outputs to Samples: SEQ2SEQVIS connects the encoder and decoder of a seq2seq model to relevant training examples by showing a neighborhood of examples with the most similar internal states. Test Alternative Decisions: SEQ2SEQVIS enables ”what if” explorations and causal relationship testing by manipulation of inputs, attention, and outputs. 


\citeA{W18-5415}: might fall under analysis techniques?

How much does “free shipping!” help an advertisement’s ability to persuade? This paper presents two methods for performance attribution: finding the degree to which an outcome can be attributed to parts of a text while controlling for potential confounders. Both algorithms are based on interpreting the behaviors and parameters of trained neural networks. One method uses a CNN to encode the text, an adversarial objective function to control for confounders, and projects its weights onto its activations to interpret the importance of each phrase towards each output class. The other method leverages residualization to control for confounds and performs interpretation by aggregating over learned word vectors. We demonstrate these algorithms’ efficacy on 118,000 internet search advertisements and outcomes, finding language indicative of high and low click through rate (CTR) regardless of who the ad is by or what it is for. Our results suggest the proposed algorithms are high performance and data efficient, able to glean actionable insights from fewer than 10,000 data points. We find that quick, easy, and authoritative language is associated with success, while lackluster embellishment is related to failure. These findings agree with the advertising industry’s emperical wisdom, automatically revealing insights which previously required manual A/B testing to discover.


\citeA{W18-5442}: no idea where to fit this, and not sure if it's really relevant to the main topic of the workshop/paper.

In this paper, we propose a method of calibrating a word embedding, so that the semantic it conveys becomes more relevant to the context. Our method is novel because the output shows clearly which senses that were originally presented in a target word embedding become stronger or weaker. This is possible by utilizing the technique of using sparse coding to recover senses that comprises a word embedding.



\citeA{W18-5449}: where should this one go?


